BehaVR: User Identification Based on VR Sensor Data

Virtual reality (VR) platforms enable a wide range of applications, however, pose unique privacy risks. In particular, VR devices are equipped with a rich set of sensors that collect personal and sensitive information (e.g., body motion, eye gaze, hand joints, and facial expression). The data from these newly available sensors can be used to uniquely identify a user, even in the absence of explicit identifiers. In this paper, we seek to understand the extent to which a user can be identified based solely on VR sensor data, within and across real-world apps from diverse genres. We consider adversaries with capabilities that range from observing APIs available within a single app (app adversary) to observing all or selected sensor measurements across multiple apps on the VR device (device adversary). To that end, we introduce BehaVR, a framework for collecting and analyzing data from all sensor groups collected by multiple apps running on a VR device. We use BehaVR to collect data from real users that interact with 20 popular real-world apps. We use that data to build machine learning models for user identification within and across apps, with features extracted from available sensor data. We show that these models can identify users with an accuracy of up to 100%, and we reveal the most important features and sensor groups, depending on the functionality of the app and the adversary. To the best of our knowledge, BehaVR is the first to analyze user identification in VR comprehensively, i.e., considering all sensor measurements available on consumer VR devices, collected by multiple real-world, as opposed to custom-made, apps.

==> references.tex <==
% Papers
@article{miller2020personal,
  title={{Personal Identifiability of User Tracking Data During Observation of 360-degree VR Video}},
  author={Miller, Mark Roman and Herrera, Fernanda and Jun, Hanseul and Landay, James A and Bailenson, Jeremy N},
  journal={Scientific Reports},
  volume={10},
  number={1},
  pages={1--10},
  year={2020},
  publisher={Springer}
}

@inproceedings{miller2022combining,
  title={{Combining Real-world Constraints on User Behavior with Deep Neural Networks for Virtual Reality (VR) Biometrics}},
  author={Miller, Robert and Banerjee, Natasha Kholgade and Banerjee, Sean},
  booktitle={2022 IEEE Conference on Virtual Reality and 3D User Interfaces (VR)},
  pages={409--418},
  year={2022},
  organization={IEEE}
}

@inproceedings{liebers2021understanding,
  title={{Understanding User Identification in Virtual Reality through Behavioral Biometrics and the Effect of Body Normalization}},
  author={Liebers, Jonathan and Abdelaziz, Mark and Mecke, Lukas and Saad, Alia and Auda, Jonas and Gruenefeld, Uwe and Alt, Florian and Schneegass, Stefan},
  booktitle={Proceedings of the 2021 CHI Conference on Human Factors in Computing Systems},
  pages={1--11},
  year={2021}
}

@inproceedings{pfeuffer2019behavioural,
  title={{Behavioural Biometrics in VR: Identifying People from Body Motion and Relations in Virtual Reality}},
  author={Pfeuffer, Ken and Geiger, Matthias J and Prange, Sarah and Mecke, Lukas and Buschek, Daniel and Alt, Florian},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
  pages={1--12},
  year={2019}
}

@inproceedings{winkler2022questsim,
  title={{QuestSim: Human Motion Tracking from Sparse Sensors with Simulated Avatars}},
  author={Winkler, Alexander and Won, Jungdam and Ye, Yuting},
  booktitle={SIGGRAPH Asia 2022 Conference Papers},
  pages={1--8},
  year={2022}
}

@article{nair2023unique,
  title={{Unique Identification of 50,000+ Virtual Reality Users from Head \& Hand Motion Data}},
  author={Nair, Vivek and Guo, Wenbo and Mattern, Justus and Wang, Rui and O'Brien, James F and Rosenberg, Louis and Song, Dawn},
  journal={arXiv preprint arXiv:2302.08927},
  year={2023}
}

@article{tricomi2022you,
  title={{You Can't Hide Behind Your Headset: User Profiling in Augmented and Virtual Reality}},
  author={Tricomi, Pier Paolo and Nenna, Federica and Pajola, Luca and Conti, Mauro and Gamberini, Luciano},
  journal={arXiv preprint arXiv:2209.10849},
  year={2022}
}

@article{de2013unique,
  title={{Unique in the Crowd: The Privacy Bounds of Human Mobility}},
  author={De Montjoye, Yves-Alexandre and Hidalgo, C{\'e}sar A and Verleysen, Michel and Blondel, Vincent D},
  journal={Scientific reports},
  volume={3},
  number={1},
  pages={1--5},
  year={2013},
  publisher={Springer}
}

@article{de2015unique,
  title={{Unique in the Shopping Mall: On the Reidentifiability of Credit Card Metadata}},
  author={De Montjoye, Yves-Alexandre and Radaelli, Laura and Singh, Vivek Kumar and Pentland, Alex “Sandy”},
  journal={Science},
  volume={347},
  number={6221},
  pages={536--539},
  year={2015},
  publisher={American Association for the Advancement of Science}
}

@inproceedings{trimananda2022ovrseen,
  title={$\{$OVRseen$\}$: Auditing Network Traffic and Privacy Policies in Oculus $\{$VR$\}$},
  author={Trimananda, Rahmadi and Le, Hieu and Cui, Hao and Ho, Janice Tran and Shuba, Anastasia and Markopoulou, Athina},
  booktitle={31st USENIX security symposium (USENIX security 22)},
  pages={3789--3806},
  year={2022}
}

@inproceedings{nair2023metaguard,
  author       = {Vivek C. Nair and
                  Gonzalo Munilla Garrido and
                  Dawn Song},
  editor       = {Sean Follmer and
                  Jeff Han and
                  J{\"{u}}rgen Steimle and
                  Nathalie Henry Riche},
  title        = {Going Incognito in the Metaverse: Achieving Theoretically Optimal
                  Privacy-Usability Tradeoffs in {VR}},
  booktitle    = {Proceedings of the 36th Annual {ACM} Symposium on User Interface Software
                  and Technology, {UIST} 2023, San Francisco, CA, USA, 29 October 2023-
                  1 November 2023},
  pages        = {61:1--61:16},
  publisher    = {{ACM}},
  year         = {2023},
  url          = {https://doi.org/10.1145/3586183.3606754},
  doi          = {10.1145/3586183.3606754},
  timestamp    = {Fri, 27 Oct 2023 20:40:55 +0200},
  biburl       = {https://dblp.org/rec/conf/uist/NairGS23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{nair2022metadata,
  title={{Exploring the Privacy Risks of Adversarial VR Game Design}},
  author={Nair, Vivek and Garrido, Gonzalo Munilla and Song, Dawn and O’Brien, James F.},
  booktitle={Proceedings on Privacy Enhancing Technologies (PoPETs)},
  year={2023}
}

@inproceedings{androidappstudy,
  author = {Enck, William and Octeau, Damien and McDaniel, Patrick and Chaudhuri, Swarat},
  title = {{A Study of Android Application Security}},
  booktitle = {{USENIX} Security},
  year = {2011},
  month = {Aug},
}

@inproceedings{ren2019information,
  title = {{Information Exposure From Consumer IoT Devices: A Multidimensional, Network-Informed Measurement Approach}},
  author = {Ren, Jingjing and Dubois, Daniel J. and Choffnes, David and Mandalari, Anna Maria and Kolcun, Roman and Haddadi, Hamed},
  booktitle = {{IMC}},
  year={2019},
}

@inproceedings{taintdroid,
  author = {William Enck and Peter Gilbert and Byung-Gon Chun and Landon P. Cox and Jaeyeon Jung and Patrick McDaniel and Anmol N. Sheth},
  title = {{TaintDroid: An Information-Flow Tracking System for Realtime Privacy Monitoring on Smartphones}},
  booktitle = {{OSDI}},
  year = {2010},
  month = {Oct},
}

@article{roesner2014security,
  title={{Security and Privacy for Augmented Reality Systems}},
  author={Roesner, Franziska and Kohno, Tadayoshi and Molnar, David},
  journal={{CACM}},
  volume={57},
  number={4},
  pages={88--96},
  year={2014},
}

@article{acquisti2014face,
  title={{Face Recognition and Privacy in the Age of Augmented Reality}},
  author={Acquisti, Alessandro and Gross, Ralph and Stutzman, Frederic D},
  journal={{Journal of Privacy and Confidentiality}},
  volume={6},
  number={2},
  pages={1},
  year={2014}
}

@book{wassom2014augmented,
  title={{Augmented Reality Law, Privacy, and Ethics: Law, Society, and Emerging AR Technologies}},
  author={Wassom, Brian},
  year={2014},
}

@article{kotsios2015privacy,
  title={{Privacy in an Augmented Reality}},
  author={Kotsios, Andreas},
  journal={{International Journal of Law and Information Technology}},
  volume={23},
  number={2},
  pages={157--185},
  year={2015},
}

@article{rauschnabel2018antecedents,
  title={{Antecedents to the Adoption of Augmented Reality Smart Glasses: A Closer Look at Privacy Risks}},
  author={Rauschnabel, Philipp A and He, Jun and Ro, Young K},
  journal={{Journal of Business Research}},
  volume={92},
  pages={374--384},
  year={2018},
}

@inproceedings{mohajeri2019watching,
  title={{Watching You Watch: The Tracking Ecosystem of Over-the-Top TV Streaming Devices}},
  author={Mohajeri Moghaddam, Hooman and Acar, Gunes and Burgess, Ben and Mathur, Arunesh and Huang, Danny Yuxing and Feamster, Nick and Felten, Edward W and Mittal, Prateek and Narayanan, Arvind},
  booktitle={{ACM CCS}},
  year={2019},
}

@inproceedings{varmarken2020tv,
  title={{The TV is Smart and Full of Trackers: Measuring Smart TV Advertising and Tracking}},
  author={Varmarken, Janus and Le, Hieu and Shuba, Anastasia and Markopoulou, Athina and Shafiq, Zubair},
  booktitle={{PETS}},
  year={2020},
}

@article{iqbal2022your,
  title={Your echos are heard: Tracking, profiling, and ad targeting in the Amazon smart speaker ecosystem},
  author={Iqbal, Umar and Bahrami, Pouneh Nikkhah and Trimananda, Rahmadi and Cui, Hao and Gamero-Garrido, Alexander and Dubois, Daniel and Choffnes, David and Markopoulou, Athina and Roesner, Franziska and Shafiq, Zubair},
  journal={arXiv preprint arXiv:2204.10920},
  year={2022}
}

@inproceedings{lentzsch2021heyalexa,
  author={Lentzsch, Christopher and Shah, Sheel Jayesh and Andow, Benjamin and Degeling, Martin and Das, Anupam and Enck, William},
  title={{Hey Alexa, is this Skill Safe?: Taking a Closer Look at the Alexa Skill Ecosystem}},
  booktitle = {NDSS},
  year={2021},
}

@inproceedings{razaghpanah2018apps,
  author    = {Abbas Razaghpanah and
               Rishab Nithyanand and
               Narseo Vallina{-}Rodriguez and
               Srikanth Sundaresan and
               Mark Allman and
               Christian Kreibich and
               Phillipa Gill},
  title     = {{Apps, Trackers, Privacy, and Regulators: A Global Study of the Mobile Tracking Ecosystem}},
  booktitle = {NDSS},
  year      = {2018},
}

@inproceedings{recon,
  author = {Ren, Jingjing and Rao, Ashwin and Lindorfer, Martina and Legout, Arnaud and Choffnes, David},
  title = {{ReCon: Revealing and Controlling PII Leaks in Mobile Network Traffic}},
  year = {2016},
  booktitle = {{MobiSys}},
}

@inproceedings{shuba2018nomoads,
	title={{NoMoAds: Effective and Efficient Cross-App Mobile Ad-Blocking}},
	author={Anastasia Shuba and Athina Markopoulou and Zubair Shafiq},
	booktitle={{PETS}},
	year={2018},
}

@inproceedings{shuba2020nomoats,
  title={{NoMoATS: Towards Automatic Detection of Mobile Tracking}},
  author={Shuba, Anastasia and Markopoulou, Athina},
  booktitle={{PETS}},
  year={2020},
}

@article{shuba2016antmonitor,
  title={{AntMonitor: A System for On-Device Mobile Network Monitoring and its Applications}}, 
  author={Anastasia Shuba and Anh Le and Emmanouil Alimpertis and Minas Gjoka and Athina Markopoulou},
  journal={arXiv preprint arXiv:1611.04268},
  year={2016}
}

@inproceedings{lebeck2018towards,
  title={{Towards Security and Privacy for Multi-User Augmented Reality: Foundations with End Users}},
  author={Lebeck, Kiron and Ruth, Kimberly and Kohno, Tadayoshi and Roesner, Franziska},
  booktitle={IEEE SP},
  year={2018},
}

@inproceedings{adams2018ethics,
  author = {Devon Adams and Alseny Bah and Catherine Barwulor and Nureli Musaby and Kadeem Pitkin and Elissa M. Redmiles},
  title = {{Ethics Emerging: the Story of Privacy and Security Perceptions in Virtual Reality}},
  booktitle = {{SOUPS}},
  year = {2018},
  month = aug,
}

@inproceedings{8802674,  
  author={Ling, Zhen and Li, Zupei and Chen, Chen and Luo, Junzhou and Yu, Wei and Fu, Xinwen},
  booktitle={{IEEE CNS}},
  title={{I Know What You Enter on Gear VR}},   
  year={2019},
}

@article{duezguen2020towards,
  title={{Towards Secure and Usable Authentication for Augmented and Virtual Reality Head-Mounted Displays}},
  author={Duezguen, Reyhan and Mayer, Peter and Das, Sanchari and Volkamer, Melanie},
  journal={arXiv preprint arXiv:2007.11663},
  year={2020}
}

@inproceedings{luooculock,
  author    = {Shiqing Luo and
               Anh Nguyen and
               Chen Song and
               Feng Lin and
               Wenyao Xu and
               Zhisheng Yan},
  title     = {{OcuLock: Exploring Human Visual System for Authentication in Virtual Reality Head-mounted Display}},
  booktitle = {NDSS},
  year      = {2020},
}

@article{garrido2023sok,
  title={SoK: Data Privacy in Virtual Reality},
  author={Garrido, Gonzalo Munilla and Nair, Vivek and Song, Dawn},
  journal={arXiv preprint arXiv:2301.05940},
  year={2023}
}

@article{paverd2014modelling,
  title={Modelling and automatically analysing privacy properties for honest-but-curious adversaries},
  author={Paverd, Andrew and Martin, Andrew and Brown, Ian},
  journal={Tech. Rep},
  year={2014}
}

@article{du2023avatars,
  title={Avatars Grow Legs: Generating Smooth Human Motion from Sparse Tracking Inputs with Diffusion Model},
  author={Du, Yuming and Kips, Robin and Pumarola, Albert and Starke, Sebastian and Thabet, Ali and Sanakoyeu, Artsiom},
  journal={arXiv preprint arXiv:2304.08577},
  year={2023}
}

% Laws
@misc{ccpa,
  author = {{State of California Department of Justice - Office of the Attorney General}},
  title = {California Consumer Privacy Act (CCPA)},
  howpublished = {\url{https://leginfo.legislature.ca.gov/faces/codes_displayText.xhtml?lawCode=CIV&division=3.&title=1.81.5.&part=4}},
  year = {2018}
}

@misc{gdpr,
  author = {European Union (EU)},
  title = {{Regulation (EU) 2016‌/679 of the European Parliament and of the Council of 27 April 2016 on the Protection of Natural Persons with Regard to the Processing of Personal Data and on the Free Movement of Such Data (General Data Protection Regulation)}},
  howpublished = {\url{https://eur-lex.europa.eu/legal-content/EN/TXT/PDF/?uri=CELEX:32016R0679}},
  year = {2018}
}

% Other books
% citation added by Ismat
@inproceedings{Ekman1978FACS,
  title={{Facial Action Coding System: Manual}},
  author={Paul Ekman and Wallace V. Friesen},
  year={1978}
}

@book{ekman2002facial,
  title={Facial Action Coding System: Facial action coding system: the manual: on CD-ROM},
  author={Ekman, Paul and Friesen, Wallace V and Hager, Joseph C},
  year={2002},
  publisher={Research Nexus}
}

% News and websites
@misc{vrgrowth,
  author = {PR Newswire},
  title = {{Virtual Reality (VR) In Healthcare Global Market Report 2023: Virtual Reality Gains Acceptance in Remote Home Assessments}},
  howpublished = {\url{https://finance.yahoo.com/news/virtual-reality-vr-healthcare-global-030000025.html}},
  year = {2023}
}

@misc{vrforeducation,
  author = {Meta},
  title = {{Our story: enter the future of learning}},
  howpublished = {\url{https://about.meta.com/immersive-learning/our-story}},
  year = {2023}
}

@misc{vrforwork,
  author = {Meta},
  title = {{Bring your teams together in Meta Horizon Workrooms}},
  howpublished = {\url{https://www.meta.com/work/workrooms/?utm_source=www.usenix.org&utm_medium=oculusredirect}},
  year = {2023}
}

@online{VR_Application,
  author    = {KnowledgeNile},
  title     = {Future Applications of Virtual Reality},
  year      = {2023},
  url       = {https://www.knowledgenile.com/blogs/future-applications-of-virtual-reality},
  urldate   = {Access Date},
}

@article{VRforFuture23,
  author       = {Pavel Smutny},
  title        = {Learning with virtual reality: a market analysis of educational and
                  training applications},
  journal      = {Interact. Learn. Environ.},
  volume       = {31},
  number       = {10},
  pages        = {6133--6146},
  year         = {2023},
  url          = {https://doi.org/10.1080/10494820.2022.2028856},
  doi          = {10.1080/10494820.2022.2028856},
  timestamp    = {Fri, 08 Mar 2024 13:22:01 +0100},
  biburl       = {https://dblp.org/rec/journals/ile/Smutny23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@misc{bodytracking,
  author = {Meta},
  title = {{This is Meta Quest Pro}},
  howpublished = {\url{https://www.meta.com/quest/quest-pro/tech-specs/}},
  year = {2023}
}

@misc{turnoffbodytracking,
  author = {Meta},
  title = {{Meta Quest Headset Tracking}},
  howpublished = {\url{https://www.meta.com/help/quest/articles/headsets-and-accessories/using-your-headset/turn-off-tracking/}},
  year = {2023}
}

@misc{handtracking,
  author = {Meta},
  title = {{Getting started with Hand Tracking on Meta Quest headsets}},
  howpublished = {\url{https://www.meta.com/help/quest/articles/headsets-and-accessories/controllers-and-hand-tracking/hand-tracking-quest-2/}},
  year = {2023}
}

@misc{eyetracking,
  author = {Meta},
  title = {{Eye tracking on Meta Quest Pro}},
  howpublished = {\url{https://www.meta.com/help/quest/articles/getting-started/getting-started-with-quest-pro/eye-tracking/}},
  year = {2023}
}

@misc{facetracking,
  author = {Meta},
  title = {{Use Natural Facial Expressions on Meta Quest Pro}},
  howpublished = {\url{https://www.meta.com/help/quest/articles/getting-started/getting-started-with-quest-pro/facial-expressions/}},
  year = {2023}
}

@misc{questpro,
  author = {Meta},
  title = {{This is Meta Quest Pro}},
  howpublished = {\url{https://www.meta.com/quest/quest-pro/}},
  year = {2023}
}

@misc{metastore,
  author = {Meta},
  title = {{Meta Quest Store}},
  howpublished = {\url{https://www.oculus.com/experiences/quest/}},
  year = {2023}
}

@misc{sidequeststore,
  author = {SIDEQUEST},
  title = {{SIDEQUEST Store}},
  howpublished = {\url{https://sidequestvr.com/}},
  year = {2023}
}

@misc{steamvrstore,
  author = {Valve},
  title = {{Steam Store}},
  howpublished = {\url{https://store.steampowered.com/}},
  year = {2023}
}

@misc{questproapi,
  author = {Meta},
  title = {{Presence Platform Introduces New Developer Tools for Meta Quest Pro}},
  howpublished = {\url{https://developer.oculus.com/blog/presence-platform-mixed-reality-social-presence-connect-2022/}},
  year = {2022}
}

@misc{androidvrpermissions,
  author = {Meta},
  title = {{Android Manifest Settings}},
  howpublished = {\url{https://developer.oculus.com/documentation/native/android/mobile-native-manifest/}},
  year = {2023}
}

@misc{steamvr,
  author = {Valve},
  title = {{SteamVR}},
  howpublished = {\url{https://store.steampowered.com/app/250820/SteamVR/}},
  year = {2023}
}

@misc{airlink,
  author = {Meta},
  title = {{Connect Meta Quest Pro or Meta Quest 2 to your PC with Air Link}},
  howpublished = {\url{https://www.meta.com/help/quest/articles/headsets-and-accessories/oculus-link/connect-with-air-link/}},
  year = {2023}
}

@misc{alvr,
  author = {ALVR},
  title = {{ALVR - Air Light VR}},
  howpublished = {\url{https://github.com/alvr-org/alvr}},
  year = {2023}
}

@misc{oculusgo,
  author = {Jacob Ridley},
  title = {{Facebook unlocks Oculus Go VR headset for developers, tinkerers, and modders}},
  howpublished = {\url{https://www.pcgamer.com/oculus-go-root-access/}},
  month = {October},
  year = {2021}
}

@misc{steamcharts,
  author = {Steam},
  title = {{CHARTS OVERVIEW}},
  howpublished = {\url{https://store.steampowered.com/charts/}},
  month = {April},
  year = {2023}
}

@misc{steamvr_user_count,
  author = {Tomislav Bezmalinovic},
  title = {{SteamVR in February 2023: PC VR usage is seemingly declining}},
  howpublished = {\url{https://mixed-news.com/en/steamvr-february-2023/}},
  month = {Feb},
  year = {2023}
}

@misc{apprankings,
  author = {SteamDB},
  title = {{Most played VR games}},
  howpublished = {\url{https://steamdb.info/charts/?tagid=21978}},
  month = {February},
  year = {2023}
}

@misc{irbminimalrisk,
  author = {US Federal Government},
  title = {{§ 46.111 Criteria for IRB approval of research (eCFR)}},
  howpublished = {\url{https://www.ecfr.gov/current/title-45/subtitle-A/subchapter-A/part-46/subpart-A/section-46.111}},
  month = {April},
  year = {2023}
}

@misc{userstatistics,
  author = {Ivan Blagojević},
  title = {{Virtual Reality Statistics}},
  howpublished = {\url{https://99firms.com/blog/virtual-reality-statistics/}},
  month = {April},
  year = {2023}
}

@misc{openxrcoordinate,
  author = {The Khronos OpenXR Working Group},
  title = {{The OpenXR Specification: § 2.16. Coordinate System}},
  howpublished = {\url{https://registry.khronos.org/OpenXR/specs/1.0/html/xrspec.html\#coordinate-system}},
  month = {April},
  year = {2023}
}

@misc{Unity_Analytics,
  author = {Unity},
  title = {{Unity Analytics}},
  howpublished = {\url{https://docs.unity.com/ugs/manual/analytics/manual/overview}},
  month = {April},
  year = {2023}
}

@misc{quaternion,
  author = {Unity},
  title = {{Quaternion}},
  howpublished = {\url{https://docs.unity3d.com/ScriptReference/Quaternion.html}},
  month = {April},
  year = {2023}
}

@misc{linearvelocity,
  author = {Unity},
  title = {{Rigidbody.velocity}},
  howpublished = {\url{https://docs.unity3d.com/ScriptReference/Rigidbody-velocity.html}},
  month = {April},
  year = {2023}
}

@misc{angularvelocity,
  author = {Unity},
  title = {{Rigidbody.angularVelocity}},
  howpublished = {\url{https://docs.unity3d.com/ScriptReference/Rigidbody-angularVelocity.html}},
  month = {April},
  year = {2023}
}

@misc{openxrstandard,
  author = {The Khronos OpenXR Working Group},
  title = {{The OpenXR Specification}},
  howpublished = {\url{https://registry.khronos.org/OpenXR/specs/1.0/html/xrspec.html}},
  month = {April},
  year = {2023}
}

@misc{openxrhandtracking,
  author = {The Khronos OpenXR Working Group},
  title = {{The OpenXR Specification: § 12.30. XR\_EXT\_hand\_tracking}},
  howpublished = {\url{https://registry.khronos.org/OpenXR/specs/1.0/html/xrspec.html\#XR_EXT_hand_tracking}},
  month = {April},
  year = {2023}
}
@misc{openxrhandjointsconvention,
  author = {The Khronos OpenXR Working Group},
  title = {{The OpenXR Specification: § 12.31.6. Conventions of hand joints}},
  howpublished = {\url{https://registry.khronos.org/OpenXR/specs/1.0/html/xrspec.html\#convention-of-hand-joints}},
  month = {April},
  year = {2023}
}

@misc{openxrfacetracking,
  author = {The Khronos OpenXR Working Group},
  title = {{The OpenXR Specification: § 12.53.7. Conventions of blend shapes}},
  howpublished = {\url{https://registry.khronos.org/OpenXR/specs/1.0/html/xrspec.html\#_conventions_of_blend_shapes}},
  month = {April},
  year = {2023}
}

@misc{openxrtoolkit,
  author = {OpenXR Toolkit Team},
  title = {{OpenXR Toolkit: Hand Tracking}},
  howpublished = {\url{https://mbucchia.github.io/OpenXR-Toolkit/hand-tracking.html}},
  month = {April},
  year = {2023}
}

@misc{eyegazepositionrotationunity,
  author = {Unity},
  title = {{Eye Gaze Interaction}},
  howpublished = {\url{https://docs.unity3d.com/Packages/com.unity.xr.openxr@1.0/manual/features/eyegazeinteraction.html}},
  month = {April},
  year = {2023}
}

@misc{eyegazepositionrotationkhronos,
  author = {The Khronos OpenXR Working Group},
  title = {{The OpenXR Specification: § 12.28. XR\_EXT\_eye\_gaze\_interaction}},
  howpublished = {\url{https://registry.khronos.org/OpenXR/specs/1.0/html/xrspec.html\#XR_EXT_eye_gaze_interaction}},
  month = {April},
  year = {2023}
}

@misc{facsexplained,
  author = {Bryn Farnsworth},
  title = {{Facial Action Coding System (FACS) – A Visual Guidebook}},
  howpublished = {\url{https://imotions.com/blog/learning/research-fundamentals/facial-action-coding-system/}},
  month = {October},
  year = {2022}
}

@misc{beatsaber,
  author = {Beat Games},
  title = {{Beat Saber}},
  howpublished = {\url{https://www.beatsaber.com/}},
  year = {2023}
}

@misc{vreyetracking,
  author = {Bryn Farnsworth},
  title = {{What is VR Eye Tracking? [And How Does it Work?]}},
  howpublished = {\url{https://imotions.com/blog/learning/best-practice/vr-eye-tracking/}},
  year = {2023}
}

@misc{BeatLeader,
  author = {Viktor Radulov},
  title = {{BeatLeader}},
  howpublished = {\url{https://www.beatleader.xyz/.}},
  month = {July},
  year = {2023}
}

@phdthesis{RF_2014,
  author       = {Gilles Louppe},
  title        = {Understanding Random Forests: From Theory to Practice},
  school       = {University of Li{\`{e}}ge, Belgium},
  year         = {2014},
  url          = {https://orbi.uliege.be/handle/2268/170309},
  timestamp    = {Mon, 31 Oct 2022 15:25:40 +0100},
  biburl       = {https://dblp.org/rec/phd/be/Louppe14.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{ShapleyFryer21,
  author       = {Daniel Vidali Fryer and
                  Inga Str{\"{u}}mke and
                  Hien D. Nguyen},
  title        = {Shapley Values for Feature Selection: The Good, the Bad, and the Axioms},
  journal      = {{IEEE} Access},
  volume       = {9},
  pages        = {144352--144360},
  year         = {2021},
  url          = {https://doi.org/10.1109/ACCESS.2021.3119110},
  doi          = {10.1109/ACCESS.2021.3119110},
  timestamp    = {Wed, 15 Dec 2021 10:28:25 +0100},
  biburl       = {https://dblp.org/rec/journals/access/FryerSN21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{SHAPLundbergL17,
  author       = {Scott M. Lundberg and
                  Su{-}In Lee},
  editor       = {Isabelle Guyon and
                  Ulrike von Luxburg and
                  Samy Bengio and
                  Hanna M. Wallach and
                  Rob Fergus and
                  S. V. N. Vishwanathan and
                  Roman Garnett},
  title        = {A Unified Approach to Interpreting Model Predictions},
  booktitle    = {Advances in Neural Information Processing Systems 30: Annual Conference
                  on Neural Information Processing Systems 2017, December 4-9, 2017,
                  Long Beach, CA, {USA}},
  pages        = {4765--4774},
  year         = {2017},
  url          = {https://proceedings.neurips.cc/paper/2017/hash/8a20a8621978632d76c43dfd28b67767-Abstract.html},
  timestamp    = {Thu, 21 Jan 2021 15:15:21 +0100},
  biburl       = {https://dblp.org/rec/conf/nips/LundbergL17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

% Behaviometrics
@article{yampolskiy2008behavioural,
  title={Behavioural biometrics: a survey and classification},
  author={Yampolskiy, Roman V and Govindaraju, Venu},
  journal={International Journal of Biometrics},
  volume={1},
  number={1},
  pages={81--113},
  year={2008},
  publisher={Inderscience Publishers}
}

@article{anjomshoa2017social,
  title={Social behaviometrics for personalized devices in the internet of things era},
  author={Anjomshoa, Fazel and Aloqaily, Moayad and Kantarci, Burak and Erol-Kantarci, Melike and Schuckers, Stephanie},
  journal={IEEE Access},
  volume={5},
  pages={12199--12213},
  year={2017},
  publisher={IEEE}
}

@inproceedings{nisenson2003towards,
  title={Towards behaviometric security systems: Learning to identify a typist},
  author={Nisenson, Mordechai and Yariv, Ido and El-Yaniv, Ran and Meir, Ron},
  booktitle={Pkdd},
  pages={363--374},
  year={2003},
  organization={Springer}
}

%Algorithms 
@Article{RF,
    title = {Classification and Regression by randomForest},
    author = {Andy Liaw and Matthew Wiener},
    journal = {R News},
    year = {2002},
    volume = {2},
    number = {3},
    pages = {18-22},
    url = {https://CRAN.R-project.org/doc/Rnews/},
  }

  @article{SVM,
  title={Support-vector networks},
  author={Cortes, Corinna and Vapnik, Vladimir},
  journal={Machine learning},
  volume={20},
  number={3},
  pages={273--297},
  year={1995},
  publisher={Springer}
}

% Privacy Policies
@misc{unity-policy,
  author = {{Unity}},
  title = {{Game Player and App User Privacy Policy}},
  howpublished = {\url{https://web.archive.org/web/20230830004711/https://unity.com/legal/game-player-and-app-user-privacy-policy}},
  month = {Aug},
  year = {2023}
}

@misc{vrchatpolicy,
  author = {VRChat Inc.},
  title = {{VRChat Privacy Policy}},
  howpublished = {\url{https://hello.vrchat.com/privacy}},
  month = {May},
  year = {2023}
}

@misc{metapolicy,
  author = {Meta Inc.},
  title = {{Supplemental Meta Platforms Technologies Privacy Policy}},
  howpublished = {\url{https://www.meta.com/legal/privacy-policy/}},
  month = {May},
  year = {2023}
}

@misc{relive_for_vr,
  author = {AMD},
  title = {{Relive for VR FAQ}},
  howpublished = {\url{https://www.amd.com/system/files/documents/amd-radeon-relive-for-vr-faq.pdf}},
  month = {May},
  year = {2024}
}

@misc{steam_link,
  author = {Valve},
  title = {{Relive for VR FAQ}},
  howpublished = {\url{https://www.meta.com/experiences/5841245619310585/}},
  month = {May},
  year = {2024}
}

@misc{meta_store,
  author = {Meta Inc.},
  title = {{Meta Store}},
  howpublished = {\url{https://www.meta.com/experiences/}},
  month = {May},
  year = {2024}
}


@article{XGB,
  title={Greedy function approximation: a gradient boosting machine},
  author={Friedman, Jerome H},
  journal={Annals of statistics},
  pages={1189--1232},
  year={2001},
  publisher={JSTOR}
}

@article{LSTM,
  added-at = {2016-11-15T08:49:43.000+0100},
  author = {Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  biburl = {https://www.bibsonomy.org/bibtex/2a4a80026d24955b267cae636aa8abe4a/dallmann},
  interhash = {0692b471c4b9ae65d00affebc09fb467},
  intrahash = {a4a80026d24955b267cae636aa8abe4a},
  journal = {Neural computation},
  keywords = {lstm rnn},
  number = 8,
  pages = {1735--1780},
  publisher = {MIT Press},
  timestamp = {2016-11-15T08:49:43.000+0100},
  title = {Long short-term memory},
  volume = 9,
  year = 1997
}




@inproceedings{MaxVote,
  author       = {Thomas G. Dietterich},
  editor       = {Josef Kittler and
                  Fabio Roli},
  title        = {Ensemble Methods in Machine Learning},
  booktitle    = {Multiple Classifier Systems, First International Workshop, {MCS} 2000,
                  Cagliari, Italy, June 21-23, 2000, Proceedings},
  series       = {Lecture Notes in Computer Science},
  volume       = {1857},
  pages        = {1--15},
  publisher    = {Springer},
  year         = {2000},
  url          = {https://doi.org/10.1007/3-540-45014-9\_1},
  doi          = {10.1007/3-540-45014-9\_1},
  timestamp    = {Tue, 14 May 2019 10:00:51 +0200},
  biburl       = {https://dblp.org/rec/conf/mcs/Dietterich00.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

% Valence
@inproceedings{suhaimi2018modeling,
  title={Modeling the affective space of 360 virtual reality videos based on arousal and valence for wearable EEG-based VR emotion classification},
  author={Suhaimi, Nazmi Sofian and Yuan, Chrystalle Tan Bih and Teo, Jason and Mountstephens, James},
  booktitle={2018 IEEE 14th International Colloquium on Signal Processing \& Its Applications (CSPA)},
  pages={167--172},
  year={2018},
  organization={IEEE}
}

@book{bouchard2011emotions,
  title={Emotions and the emotional valence afforded by the virtual environment},
  author={Bouchard, St{\'e}phane and Labont{\'e}-Chartrand, G},
  year={2011},
  publisher={IntechOpen}
}

% Human factors (agency and emotions)
@inproceedings{jicol2023realism,
  title={Realism and Field of View Affect Presence in VR but Not the Way You Think},
  author={Jicol, Crescent and Clarke, Christopher and Tor, Emilia and Dakin, Rebecca M and Lancaster, Tom Charlie and Chang, Sze Tung and Petrini, Karin and O'Neill, Eamonn and Proulx, Michael J and Lutteroth, Christof},
  booktitle={Proceedings of the 2023 CHI Conference on Human Factors in Computing Systems},
  pages={1--17},
  year={2023}
}

@article{kuppens2013relation,
  title={The relation between valence and arousal in subjective experience.},
  author={Kuppens, Peter and Tuerlinckx, Francis and Russell, James A and Barrett, Lisa Feldman},
  journal={Psychological bulletin},
  volume={139},
  number={4},
  pages={917},
  year={2013},
  publisher={American Psychological Association}
}

% Vision Pro
@misc{visionproapple,
  author = {Apple Inc.},
  title = {{Vision Pro}},
  howpublished = {\url{https://www.apple.com/apple-vision-pro/}},
  month = {June},
  year = {2023}
}

@misc{visionproblog,
  author = {Yash and Jibin},
  title = {{Apple Vision Pro features, specs, price, and release date}},
  howpublished = {\url{https://www.igeeksblog.com/apple-vision-pro-features/}},
  month = {June},
  year = {2023}
}


@article{olade2020biomove,
  title={Biomove: Biometric user identification from human kinesiological movements for virtual reality systems},
  author={Olade, Ilesanmi and Fleming, Charles and Liang, Hai-Ning},
  journal={Sensors},
  volume={20},
  number={10},
  pages={2944},
  year={2020},
  publisher={MDPI}
}

%--------Extra related work---------------------------------------------------------------------------------

@inproceedings{kaleido_USENIX21,
  author       = {Jingjie Li and
                  Amrita Roy Chowdhury and
                  Kassem Fawaz and
                  Younghyun Kim},
  editor       = {Michael Bailey and
                  Rachel Greenstadt},
  title        = {Kal{\(\epsilon\)}ido: Real-Time Privacy Control for Eye-Tracking Systems},
  booktitle    = {30th {USENIX} Security Symposium, {USENIX} Security 2021, August 11-13,
                  2021},
  pages        = {1793--1810},
  publisher    = {{USENIX} Association},
  year         = {2021},
  url          = {https://www.usenix.org/conference/usenixsecurity21/presentation/li-jingjie},
  timestamp    = {Thu, 28 Oct 2021 08:30:13 +0200},
  biburl       = {https://dblp.org/rec/conf/uss/Li0FK21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{VREED21,
  author       = {Luma Tabbaa and
                  Ryan Searle and
                  Saber Mirzaee Bafti and
                  Md. Moinul Hossain and
                  Jittrapol Intarasirisawat and
                  Maxine Glancy and
                  Chee Siang Ang},
  title        = {{VREED:} Virtual Reality Emotion Recognition Dataset Using Eye Tracking
                  {\&} Physiological Measures},
  journal      = {Proc. {ACM} Interact. Mob. Wearable Ubiquitous Technol.},
  volume       = {5},
  number       = {4},
  pages        = {178:1--178:20},
  year         = {2021},
  url          = {https://doi.org/10.1145/3495002},
  doi          = {10.1145/3495002},
  timestamp    = {Fri, 06 May 2022 13:46:21 +0200},
  biburl       = {https://dblp.org/rec/journals/imwut/TabbaaSBHIGA21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{EmotionPD2019,
  title={Measuring emotion recognition by people with Parkinson’s disease using eye-tracking with dynamic facial expressions},
  author={Judith Bek and Ellen Poliakoff and Karen Lander},
  journal={Journal of Neuroscience Methods},
  year={2019},
  volume={331},
  url={https://api.semanticscholar.org/CorpusID:208069560}
}

@inproceedings{stephenson2022sok,
  title={Sok: Authentication in augmented and virtual reality},
  author={Stephenson, Sophie and Pal, Bijeeta and Fan, Stephen and Fernandes, Earlence and Zhao, Yuhang and Chatterjee, Rahul},
  booktitle={2022 IEEE Symposium on Security and Privacy (SP)},
  pages={267--284},
  year={2022},
  organization={IEEE}
}

% Number of VR apps
@misc{steamvrnumberofapps,
  author = {Steam},
  title = {{Virtual Reality Titles}},
  howpublished = {\url{https://store.steampowered.com/vr}},
  month = {July},
  year = {2023}
}

@misc{metaquestnumberofapps,
  author = {Tomislav Bezmalinovic},
  title = {{Meta Quest Store: 5 Things You (Probably) Didn't Know}},
  howpublished = {\url{https://mixed-news.com/en/meta-quest-store-analysis/}},
  month = {April},
  year = {2023}
}

% Tracking in various ecosystems
@inproceedings{degeling2018we,
  title={We value your privacy... now take some cookies: Measuring the GDPR's impact on web privacy},
  author={Degeling, Martin and Utz, Christine and Lentzsch, Christopher and Hosseini, Henry and Schaub, Florian and Holz, Thorsten},
  booktitle = {{NDSS}},
  year={2019},
}

% Biometrics
@article{boutros2020iris,
  title={Iris and periocular biometrics for head mounted displays: Segmentation, recognition, and synthetic data generation},
  author={Boutros, Fadi and Damer, Naser and Raja, Kiran and Ramachandra, Raghavendra and Kirchbuchner, Florian and Kuijper, Arjan},
  journal={Image and Vision Computing},
  volume={104},
  pages={104007},
  year={2020},
  publisher={Elsevier}
}


@article{VRforTrainingSH21,
  author       = {Alexandra D. Kaplan and
                  Jessica Cruit and
                  Mica R. Endsley and
                  Suzanne M. Beers and
                  Ben D. Sawyer and
                  Peter A. Hancock},
  title        = {The Effects of Virtual Reality, Augmented Reality, and Mixed Reality
                  as Training Enhancement Methods: {A} Meta-Analysis},
  journal      = {Hum. Factors},
  volume       = {63},
  number       = {4},
  year         = {2021},
  url          = {https://doi.org/10.1177/0018720820904229},
  doi          = {10.1177/0018720820904229},
  timestamp    = {Sat, 31 Jul 2021 17:22:07 +0200},
  biburl       = {https://dblp.org/rec/journals/hf/KaplanCEBSH21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{IEEEVRMeusum19,
  author       = {David A. Plecher and
                  Maximilian Wandinger and
                  Gudrun Klinker},
  title        = {Mixed Reality for Cultural Heritage},
  booktitle    = {{IEEE} Conference on Virtual Reality and 3D User Interfaces, {VR}
                  2019, Osaka, Japan, March 23-27, 2019},
  pages        = {1618--1622},
  publisher    = {{IEEE}},
  year         = {2019},
  url          = {https://doi.org/10.1109/VR.2019.8797846},
  doi          = {10.1109/VR.2019.8797846},
  timestamp    = {Mon, 15 Jun 2020 17:10:17 +0200},
  biburl       = {https://dblp.org/rec/conf/vr/PlecherWK19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@online{metaquest_policy,
    author = {Meta},
    title = {App Privacy Data Types on Meta Quest},
    year = {Accessed: 2024},
    url = {https://www.meta.com/help/quest/articles/accounts/privacy-information-and-settings/app-privacy-data-types-meta-quest/}
}

@inproceedings{radway_permissionOculus23,
    author = {Radway, Sarah and Votipka, Daniel},
    title = {Identifying New Challenges In The Oculus Permissions Framework},
    booktitle = {Proceedings of the Symposium On Usable Privacy and Security (SOUPS) 2023, Poster Session},
    organization = {USENIX Association},
    year = {2023},
}

@article{Ensemble_GanaieHMTS22,
  author       = {M. A. Ganaie and
                  Minghui Hu and
                  Ashwani Kumar Malik and
                  Muhammad Tanveer and
                  Ponnuthurai N. Suganthan},
  title        = {Ensemble deep learning: {A} review},
  journal      = {Eng. Appl. Artif. Intell.},
  volume       = {115},
  pages        = {105151},
  year         = {2022},
  url          = {https://doi.org/10.1016/j.engappai.2022.105151},
  doi          = {10.1016/J.ENGAPPAI.2022.105151},
  timestamp    = {Sat, 05 Aug 2023 00:02:13 +0200},
  biburl       = {https://dblp.org/rec/journals/eaai/GanaieHMTS22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@misc{steam_vr_app_count,
  author = {SteamDB},
  title = {{SteamDB -- Tags: VR (Archive.is snapshot)}},
  howpublished = {\url{http://archive.today/2024.05.22-164720/https://steamdb.info/tag/21978/}},
  month = {May},
  year = {2024}
}

@misc{quest_sale_count,
  author = {Alex Heath},
  title = {{This is Meta’s AR / VR hardware roadmap through 2027}},
  howpublished = {\url{https://www.theverge.com/2023/2/28/23619730/meta-vr-oculus-ar-glasses-smartwatch-plans}},
  month = {May},
  year = {2024}
}

@article{privacyNudges_online17,
  author       = {Alessandro Acquisti and
                  Idris Adjerid and
                  Rebecca Balebako and
                  Laura Brandimarte and
                  Lorrie Faith Cranor and
                  Saranga Komanduri and
                  Pedro Giovanni Leon and
                  Norman M. Sadeh and
                  Florian Schaub and
                  Manya Sleeper and
                  Yang Wang and
                  Shomir Wilson},
  title        = {Nudges for Privacy and Security: Understanding and Assisting Users'
                  Choices Online},
  journal      = {{ACM} Comput. Surv.},
  volume       = {50},
  number       = {3},
  pages        = {44:1--44:41},
  year         = {2017},
  url          = {https://doi.org/10.1145/3054926},
  doi          = {10.1145/3054926},
  timestamp    = {Sat, 09 Apr 2022 12:27:18 +0200},
  biburl       = {https://dblp.org/rec/journals/csur/AcquistiABBCKLS17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{privacyrecommendation_widard10,
  author       = {Lujun Fang and
                  Heedo Kim and
                  Kristen LeFevre and
                  Aaron Tami},
  editor       = {Ehab Al{-}Shaer and
                  Angelos D. Keromytis and
                  Vitaly Shmatikov},
  title        = {A privacy recommendation wizard for users of social networking sites},
  booktitle    = {Proceedings of the 17th {ACM} Conference on Computer and Communications
                  Security, {CCS} 2010, Chicago, Illinois, USA, October 4-8, 2010},
  pages        = {630--632},
  publisher    = {{ACM}},
  year         = {2010},
  url          = {https://doi.org/10.1145/1866307.1866378},
  doi          = {10.1145/1866307.1866378},
  timestamp    = {Tue, 10 Nov 2020 20:00:21 +0100},
  biburl       = {https://dblp.org/rec/conf/ccs/FangKLT10.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{GuoDLZXH24_userRecommendation,
  author       = {Hanyang Guo and
                  Hong{-}Ning Dai and
                  Xiapu Luo and
                  Zibin Zheng and
                  Gengyang Xu and
                  Fengliang He},
  title        = {An Empirical Study on Oculus Virtual Reality Applications: Security
                  and Privacy Perspectives},
  booktitle    = {Proceedings of the 46th {IEEE/ACM} International Conference on Software
                  Engineering, {ICSE} 2024, Lisbon, Portugal, April 14-20, 2024},
  pages        = {159:1--159:13},
  publisher    = {{ACM}},
  year         = {2024},
  url          = {https://doi.org/10.1145/3597503.3639082},
  doi          = {10.1145/3597503.3639082},
  timestamp    = {Wed, 22 May 2024 14:55:20 +0200},
  biburl       = {https://dblp.org/rec/conf/icse/GuoDLZXH24.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@book{dwork2006differential,
  author    = {Cynthia Dwork},
  title     = {Differential Privacy},
  year      = {2006},
  publisher = {Springer},
  address   = {Berlin},
  note      = {Tutorial presentation at the International Conference on Automata, Languages and Programming (ICALP)}
}

#Feature Selection
@article{guyon2003feature,
  title={An introduction to variable and feature selection},
  author={Guyon, Isabelle and Elisseeff, Andr{\'e}},
  journal={Journal of Machine Learning Research},
  volume={3},
  number={Mar},
  pages={1157--1182},
  year={2003}
}

@article{singh2021feature,
  title={Feature selection methods in data mining: A comparative study},
  author={Singh, Hardeep and Singh, Gurvinder},
  journal={Materials Today: Proceedings},
  volume={47},
  number={2},
  pages={204-208},
  year={2021},
  publisher={Elsevier}
}


